Stylized Meta-Album: Group-bias injection with style transfer to study robustness against distribution shifts

We introduce Stylized Meta-Album (SMA), a new image classification meta-dataset comprising 24 datasets (12 content datasets, and 12 stylized datasets), designed to advance studies on out-of-distribution (OOD) generalization and related topics. Created using style transfer techniques from 12 subject classification datasets, SMA provides a diverse and extensive set of 4800 groups, combining various subjects (objects, plants, animals, human actions, textures) with multiple styles. SMA enables flexible control over groups and classes, allowing us to configure datasets to reflect diverse benchmark scenarios. While ideally, data collection would capture extensive group diversity, practical constraints often make this infeasible. SMA addresses this by enabling large and configurable group structures through flexible control over styles, subject classes, and domains-allowing datasets to reflect a wide range of real-world benchmark scenarios. This design not only expands group and class diversity, but also opens new methodological directions for evaluating model performance across diverse group and domain configurations-including scenarios with many minority groups, varying group imbalance, and complex domain shifts-and for studying fairness, robustness, and adaptation under a broader range of realistic conditions. To demonstrate SMA's effectiveness, we implemented two benchmarks: (1) a novel OOD generalization and group fairness benchmark leveraging SMA's domain, class, and group diversity to evaluate existing benchmarks. Our findings reveal that while simple balancing and algorithms utilizing group information remain competitive as claimed in previous benchmarks, increasing group diversity significantly impacts fairness, altering the superiority and relative rankings of algorithms. We also propose to use \textit{Top-M worst group accuracy} as a new hyperparameter tuning metric, demonstrating broader fairness during optimization and delivering better final worst-group accuracy for larger group diversity. (2) An unsupervised domain adaptation (UDA) benchmark utilizing SMA's group diversity to evaluate UDA algorithms across more scenarios, offering a more comprehensive benchmark with lower error bars (reduced by 73\% and 28\% in closed-set setting and UniDA setting, respectively) compared to existing efforts. These use cases highlight SMA's potential to significantly impact the outcomes of conventional benchmarks.

==> appendices/style-transfer-algorithm.tex <==
\section{Neural Style Transfer algorithm}


\label{appendix:neural-style-transfer-algorithm}



For our style transfer, we used VGG-19 to reconstruct the \textit{style} and \textit{content} of input images in the following steps:
\begin{itemize}
\item First, it generates a white noise image as initialization called \textit{generated image}.
\item Then, both the \textit{content image} and the \textit{generated image} are passed through the pre-trained VGG-19 model. The squared-error content loss between the two feature representations is then defined:
\begin{equation}
L_{content} = \sum_{l=0}^L w_l \left[ \sum_{ij} (F_{ij}^l - P_{ij}^l)^2 \right]
\end{equation}

where $F^l$ is the output of \textit{content image} at layers $l$, $P^l$ is the output of \textit{generated image} at layers $l$ and $w_l$ is the weight for each layer indicating how much a layer contributes to the content loss
\item To reconstruct style, we also pass both the style image and generated image through VGG-19. The squared-error style loss between the two feature representations is then defined:
\begin{equation}
L_{style} = \sum_{l=0}^L \left[\frac{w_l}{4N_l^2M_l^2} \sum_{ij} (G_{ij}^l - A_{ij}^l)^2\right]
\end{equation}

where $A^l$ is the Gram matrix of the output of \textit{generated image} at layers $l$, $G^l$ is the Gram matrix of the output of \textit{style image} at layers $l$, $w_l$ is the weight indicating the degree to which that layer contributes to the style loss, $N_l$ is the number of channels of that layer, and $M_l$ is the total number of features - the product of the channel's height and width - for each channel of that layer.

\item Finally, we minimize the total loss function:
\begin{equation}
L_{total} = \alpha L_{content} + \beta L_{style}
\end{equation}
% with $\frac{\beta}{\alpha}=100$ and using L-BFGS as optimizer because we get the best results from these particular settings.

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figs/styletransfer_algo_summarization.png}
    \caption{Style Transfer Algorithm summarization}
    \label{fig:stf-algo-summarize}
\end{figure}

\end{itemize}


By experiments, we will use the following layers to calculate the losses of Neural Style Transfer:
 conv1\_1, conv2\_1, conv3\_1, conv4\_1, and conv5.

==> appendices/style-transfer.tex <==
\section{Style Transfer}
\label{appendix:style-transfer}


We used Neural Style Transfer\cite{gatys2015neural} to introduce a different protected attribute to our dataset called \textit{style}. This \textit{style} attribute will then be used as a controlled nuisance factor Z to conduct in-depth analyses of the impact of bias in data on the generalization of several baseline methods.

Similar to the original version of Neural Style Transfer \cite{gatys2015neural}, we used VGG-19 to reconstruct the \textit{style} and \textit{content} of input images. The following parameters give the best results in our experiments:

\begin{itemize}
\item Optimizer: L-BFGS
\item Chosen layers for final loss calculation:
 conv1\_1, conv2\_1, conv3\_1, conv4\_1, and conv5
\item $\frac{\beta}{\alpha}=100$, where $\alpha$ and $\beta$ are the weights of the final loss function:
\begin{equation}
L_{total} = \alpha L_{content} + \beta L_{style}
\end{equation}
\end{itemize}


==> sections/_submission_info.tex <==
% Submission information
\section*{Submission Information: TO BE DELETED}
% 
% \begin{itemize}
    \item Submission Date: mid-April 2024
    \item Conference/Journal: \url{https://data.mlr.press}
    \item Submission information page: \url{https://data.mlr.press/submissions}
    \item In particular, submissions introducing new datasets must follow the dataset submission guidelines of NeurIPS Datasets and Benchmarks by including the following in the supplementary materials (as a separate PDF): 1) Dataset documentation and intended uses. 2) URL to website/platform where the dataset/benchmark can be viewed and downloaded by the reviewers. 3) Author statement that they bear all responsibility in case of violation of rights, etc., and confirmation of the data license. 4) Hosting, licensing, and maintenance plan. 
    \item No page limitation in general
    }
\end{itemize}


==> sections/checklist.tex <==
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope? 
  \answerYes{}
  \item Did you describe the limitations of your work? 
  \answerYes{See Section~\ref{sec:Illustrative-Use-Case-Group-Fairness}, Section~\ref{sec:Discussion-and-conclusion}.} 
  \item Did you discuss any potential negative societal impacts of your work? 
  \answerNA{There are no negative societal impacts. Rather, this meta-dataset can foster progress in the fields of out-of-distribution generalization and fairness. We have added ``recommended use'' in Section \ref{sec:contributions}.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}

	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (\eg for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
  \answerYes{The code and instructions are publicly released on the Meta-Album GitHub repository (\url{https://github.com/stylized-meta-album/code})}
  \item Did you specify all the training details (\eg data splits, hyperparameters, how they were chosen)?\\
    \answerYes{See Section \ref{sec:Illustrative-Use-Case-Group-Fairness}. Additional details can be found in the Stylized-Meta-Album GitHub repository.}
	\item Did you report error bars (\eg with respect to the random seed after running experiments multiple times)?
    \answerYes{See Table~\ref{tab:use-case-group-fairness-results}, Figure~\ref{fig:template-verification},
    }
	\item Did you include the total amount of compute and the type of resources used (\eg type of GPUs, internal cluster, or cloud provider)?
	\answerYes{See Section \ref{sec:Illustrative-Use-Case-Group-Fairness}}

\end{enumerate}

\item If you are using existing assets (\eg code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?\\
    \answerYes{See 
    Section~\ref{sec:Illustrative-Use-Case-Group-Fairness}, Section~\ref{sub-sec:style-transfer}}

  \item Did you mention the license of the assets?\\
    \answerYes{See Section~\ref{sub-sec:release} and Appendix~\ref{appendix:license}}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{We provide software for data scraping, and data formatting on the Github repository \url{https://github.com/stylized-meta-album/code}}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
  \answerYes{Our meta-dataset is based on Meta-Album which is open for non-commercial use.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{None of the datasets allow for personal identification}

\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> tables/comparison-of-multi-source-benchmarks.tex <==
\begin{table}[t]
  \caption{\textbf{Comparison between SMA and other multi-source benchmarks}.}
  \label{tab:comparison-of-multi-source-benchmarks}
  \centering
  \begin{adjustbox}{width=\linewidth}
  \begin{tabular}{l r r r r r r c c c}
    \toprule
    \makecell{Dataset} & 
    \multicolumn{1}{c}{\rot{\# of images}} & 
    \rot{\# of classes} & 
    \rot{\# of sources}  & 
    \multicolumn{1}{c}{\rot{\makecell{min/max images\\per class}}}  &
    \multicolumn{1}{c}{\rot{\makecell{min/max images\\per source}}} &
    \multicolumn{1}{c}{\rot{\makecell{min/max classes\\per source}}} &
    \multicolumn{1}{c}{\rot{\makecell{multi-datasets}}} & 
    \multicolumn{1}{c}{\rot{\makecell{multi-versions}}} & 
    \multicolumn{1}{c}{\rot{\makecell{uniform image\\size}}} \\
    \midrule
    Office-Home \cite{OfficeHome} & $15\,588$ & 65 & 4 & $142\,/\,363$ & $2\,427\,/\,4\,439$ & $65\,/\,65$ & \xmark & \xmark & \xmark 
    \\
    PACS \cite{PACS} & $9\,991$ & 7 & 4 & $943\,/\,1\,729$ & $1\,670\,/\,3\,929$ & $7\,/\,7$ & \xmark & \xmark & \cmark 
    \\
    DomainNet \cite{DomainNet} & $596\,006$ & 345 & 6 & $878\,/\,2\,799$ & $48\,833\,/\,175\,327$ & $345\,/\,345$ & \xmark & \xmark & \xmark
    \\
    ImageNet-R \cite{ImageNet-R} & $30\,000$ & 200 & 15 & $51\,/\,430$ & $508\,/\,5\,673$ & $106\,/\,200$ & \xmark & \xmark & \xmark 
    \\
    \textbf{Stylized Meta-Album} & $\mathbf{4\,677\,000}$ & \textbf{220} & \textbf{20} & $\mathbf{56\,/\,6101}$ & $\mathbf{1\,395\,/\,97\,797}$ & $\mathbf{200\,/\,200}$ & \cmark & \cmark & \cmark
    \\
    \bottomrule
  \end{tabular}
  \end{adjustbox}
\end{table}
